PCMPC: Perception-Constrained Model Predictive Control for Quadrotors with Suspended Loads using a Single Camera and IMU

In this paper, we address the Perception--Constrained Model Predictive Control (PCMPC) and state estimation problems for quadrotors with cable suspended payloads using a single camera and Inertial Measurement Unit (IMU). We design a receding--horizon control strategy for cable suspended payloads directly formulated on the system manifold configuration space SE(3)xS^2. The approach considers the system dynamics, actuator limits and the camera's Field Of View (FOV) constraint to guarantee the payload's visibility during motion. The monocular camera, IMU, and vehicle's motor speeds are combined to provide estimation of the vehicle's states in 3D space, the payload's states, the cable's direction and velocity. The proposed control and state estimation solution runs in real-time at 500 Hz on a small quadrotor equipped with a limited computational unit. The approach is validated through experimental results considering a cable suspended payload trajectory tracking problem at different speeds.

==> symbol_list.tex <==
%!TEX root = ARTICLE.tex
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathOperator{\Diag}{Diag} 
%%%%%%%%%%%%% Comando para glosario %%%%%%%%%%%%%%55
\newcommand{\glo}[3]{
%#1: id
%#2: name
%#3: 
	\newglossaryentry{#1}
	{
	  name=#2,
	  description=#3,
	}
}
%%%%%%%%%%%%%%% Comando para definir un simbolo%%%%
\newcommand{\glom}[4]{
%#1: id
%#2: name
%#2: Symbol
%#3: description
	\newglossaryentry{#1}
	{
	  name={\ensuremath{#2}},
	  symbol={\ensuremath{#3}},
	  description=#4,
	  type=symbols,
	}
}
%%%%%%%%%%%%%%% Comando para definir un simbolo%%%%
\newcommand{\glomh}[4]{
%#1: id
%#2: name
%#2: Symbol
%#3: description
	\newglossaryentry{#1}
	{
	  name={\ensuremath{#2}},
	  symbol={\ensuremath{#3}},
	  description=#4,
	  %type=hidden,
	}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\glo{naiive}{naive}{ratio of circumference of circle to its
               diameter}



%%http://tex.stackexchange.com/questions/236670/custom-glossary-style-makenoidxglossaries-and-glsgroupskip


%% Linear model
\glomh{linx}{A}{A}{Input matrix.}
\glomh{linp}{C}{C}{parameter matrix.}


% dynamics
\glom{sgn}{\chi}{\chi}{Indicator function}
\glom{error}{e}{e}{Desired roll}
% \glom{droll}{\phi^*}{\phi^*}{Desired roll}
\glom{roll}{\phi}{\phi}{roll}
\glom{pitch}{\theta}{\theta}{pitch}
\glom{yaw}{\psi}{\psi}{yaw}
\glom{droll}{ p}{ p}{roll}
\glom{dpitch}{ q}{ q}{pitch}
\glom{dyaw}{ r}{ r}{yaw}
\glom{angles}{\mathbf{\Theta}}{\mathbf{\Theta}}{Robot attitude}
\glom{dangles}{\mathbf{\Omega}}{\mathbf{\Omega}}{Angular velocities}
\glom{id}{k}{k}{general id of robot used in description of control method and estimation}

\glom{thrust}{F}{F}{Thrust}
\glom{u}{\mathbf{u}}{\mathbf{u}}{control input}
\glom{w}{\mathbf{w}}{\mathbf{w}}{control input}
\glom{angular}{\omega}{\omega}{angular speed}

% Coordinate frames
\glom{worldf}{\mathcal{I}}{\mathcal{I}}{World frame}
\glom{loadf}{\mathcal{L}}{\mathcal{L}}{Load frame}
\glom{robotf}{\mathcal{B}}{\mathcal{B}}{Body frame}
\glom{camf}{\mathcal{C}}{\mathcal{C}}{Camera frame}

%\glom{tagf}{\mathpzc{T}}{\mathpzc{T}}{Tag frame}
%\glom{dockf}{\mathpzc{d}}{\mathpzc{d}}{Docking module frame}
%\glom{camf}{\mathpzc{C}}{\mathpzc{C}}{Camera frame}
%\glom{waitf}{\mathpzc{w}}{\mathpzc{w}}{Waiting module frame}

%% Robots
\glom{tag}{\mathpzc{t}_p}{\mathpzc{t}_p}{Tag}
\glom{robots}{\mathcal{R}}{\mathcal{R}}{Set of a team of robots}
\glom{robotl}{\mathbf{x}}{\mathbf{x}}{Robot location.}
\glom{robot}{\mathbf{x}}{\mathbf{x}}{Robot location.}
\glom{width}{\mathpzc{w}}{\mathpzc{w}}{Robot width.}
\glom{height}{\mathpzc{h}}{\mathpzc{h}}{Robot height.}
\glom{orientations}{\Psi}{\Psi}{Robot orientations.}
\glom{orientation}{\psi}{\psi}{Robot orientation.}
\glom{structure}{\mathit{S}}{\mathit{S}}{Structure}
\glom{structureset}{\mathcal{S_F}}{\mathcal{S_F}}{Structure set}
\glom{component}{\mathit{S}}{\mathit{S}}{Structure}

% Desired structure
\glom{targets}{\mathcal{Z}}{\mathcal{Z}}{Target points}
\glom{targetse}{\mathcal{Z}^E}{\mathcal{Z}^E}{Expanded target points}
\glom{target}{z}{z}{Robot location.}

\glom{tree}{\mathcal{T}}{\mathcal{T}}{Assembly tree.}
\glom{tedges}{\mathcal{E}^\mathcal{T}}{\mathcal{E}^\mathcal{T}}{Edges of the Assembly tree.}
\glom{tvertices}{\mathcal{V}^\mathcal{T}}{\mathcal{V}^\mathcal{T}}{Vertices of the Assembly tree.}
\glom{tivertices}{\mathcal{V}^{\mathcal{T}_i}}{\mathcal{V}^{\mathcal{T}_i}}{Vertices of the Assembly tree.}

\glom{graph}{\mathcal{G}}{\mathcal{G}}{Communication graph}
\glom{cgraph}{\hat{\mathcal{G}}}{\hat{\mathcal{G}}}{Canonical robust graph}
\glom{vertices}{\mathcal{V}}{\mathcal{V}}{Set of Vertices}
\glom{neighbors}{\mathcal{N}_i}{\mathcal{N}}{Neighbors for node $i$}
\glom{edges}{\mathcal{E}}{\mathcal{E}}{Set of Edges}
\glom{neighborsi}{\mathcal{J}_i}{\mathcal{J}}{Inclusive Neighbors for node $i$}
\glom{removed}{\mathcal{R}}{\mathcal{R}}{Removed nodes}
\glom{normal}{\mathcal{N}}{\mathcal{N}}{Normal nodes}
\glom{strongset}{\mathcal{F}}{\mathcal{F}}{Strong nodes}
\glom{weakset}{\mathcal{W}}{\mathcal{W}}{Weak nodes}
\glom{candidates}{\mathcal{C}}{\mathcal{C}}{Candidate points}
\glom{boundary}{\mathcal{P}}{\mathcal{P}}{Objective points}

\glom{loc}{v}{v}{Node location in the space}
\glom{val}{x}{x}{Variable of interest of the node}

\glom{received}{\mathcal{P}_i^t}{\mathcal{P}}{Set of received values by node $i$ a the time interval 
%$[t-T\, t]$
}


